Orientation-aware Semantic Segmentation on Icosahedron Spheres

We address semantic segmentation on omnidirectional images, to leverage a holistic understanding of the surrounding scene for applications like autonomous driving systems. For the spherical domain, several methods recently adopt an icosahedron mesh, but systems are typically rotation invariant or require significant memory and parameters, thus enabling execution only at very low resolutions. In our work, we propose an orientation-aware CNN framework for the icosahedron mesh. Our representation allows for fast network operations, as our design simplifies to standard network operations of classical CNNs, but under consideration of north-aligned kernel convolutions for features on the sphere. We implement our representation and demonstrate its memory efficiency up-to a level-8 resolution mesh (equivalent to 640 x 1024 equirectangular images). Finally, since our kernels operate on the tangent of the sphere, standard feature weights, pretrained on perspective data, can be directly transferred with only small need for weight refinement. In our evaluation our orientation-aware CNN becomes a new state of the art for the recent 2D3DS dataset, and our Omni-SYNTHIA version of SYNTHIA. Rotation invariant classification and segmentation tasks are additionally presented for comparison to prior art.

==> sections/old_stuff.tex <==
%\section{Introduction}
%Omnidirectional images offer full field of view and are seen most suitable in areas such as virtual reality, robotics, and autonomous vehicle. Image acquisition from a wider field of view could improve the performance of many computer vision tasks such as visual odometry \cite{zhang2016benefit}. However, omnidirectional images are often represented with equirectangular projection to linearly map spherical coordinates to image plane. The mapping will inevitably result distortions at different elevations, especially near polar areas. Therefore, the regular Convolutional Neural Networks (CNNs) will only achieve non-optimal performance if applied directly on equirectangular images. Moreover, learnable filters could not be shared at different polar angles due to the distortions. 
%Instead of dealing with equirectangular images or cube maps, we propose to work on spherical mesh which is a natural representation of omnidirectional images. The representation is preferred to alternatives due to its minimal distortion and inherent continuity. Furthermore, the property of parameter sharing could be nicely kept similarly as is to perspective images to make the network efficient. Through this work, we assume the captured images have dominant upright orientation. By further taking advantage of the multilevel subdivision nature, pooling operations become simple and efficient to implement for spherical mesh. 

%In this work, we propose to represent omnidirectional images in spherical mesh and develop convolution, pooling and up-sampling operators accordingly. The resulting network called ``hexNet" is performed on image classification  and semantic segmentation tasks. 

%\section{Related work}
%The work is mostly related to \cite{lee2018spherephd} in which the spherical polyhedron representation is used. To deal with vertices lying in pentagons and hexagons, the filter kernel is designed to work on triangular pixels/faces rather than vertices. Experiments on rotated MNIST classification and SYNTHIA vehicle detection show that the proposed representation outperforms equirectangular images and cube maps. However, the filters have to be flipped to handle adjacent faces. There is no semantic segmentation results provided either.

%\paragraph{Graph-based CNNs:}
%\cite{khasanova2017graph, defferrard2016convolutional}. Khasanova \etal \cite{khasanova2017graph} propose a novel image classification method based on deep neural network designed for omnidirectional cameras. The graph construction method allows learning filters that respond similarly to objects distortion at different elevations. Defferrard \etal \cite{defferrard2016convolutional} present a formulation of CNNs in the context of spectral graph theory to design fast localized convolutional filters on graphs. For both methods, experiments on omni-MNIST demonstrate the effectiveness. 

%\paragraph{Spherical CNNs:}
%Cohen \etal \cite{cohen2018spherical} propose to encode rotation equivariance using spherical CNNs. Generalized Fourier transform and fast version for sphere and rotation group are introduced. However, it is not clear how to integrate the method for more complex vision tasks. Esteves \etal \cite{esteves2018learning} used spherical harmonic basis to achieve similar results. Zhou \etal \cite{zhou2017oriented} propose to extend normal CNNs to include an additional channel for orientations to extract rotation-dependent features from images. 

%\paragraph{CNNs with adapted kernels:}
%Another line of work aims to adapt the regular grid kernel to work with omnidirectional images.
%Su \& Grauman \cite{su2017learning} propose to treat equirectangular images as perspective ones by adapting the weights according to the elavations. The method aims to minimize the error of intermediate layers between the classic CNNs and the one using equirectangular as input. Independently, both Zhao \etal \cite{zhao2018distortion} and Coors \etal \cite{coors2018spherenet} proposed the idea of distorting rectangular convolution kernels. 

%\paragraph{Reparameterized Convolutional Kernel:}
%Several works utilize the diffusion kernel for efficient CNNs. Kondor and Lafferty \cite{kondor2002diffusion} was among the first to suggest using diffusion kernel on graphs. Boscani \etal \cite{boscaini2016learning} generalizes CNNs to non-Euclidean domain by using a set of oriented anisotropic diffusion kernels. Cohen and Welling \cite{cohen2016steerable} utilized a linear combinations of filter banks to acquire equivariant convolution filters. Jiang \etal \cite{jiang2018spherical} propose to use linear combinations of parameterized differential operators to replace cross-correlation. The network has much less parameters since each kernel only have 4 scalar numbers. However, the proposed MeshCOV layer could only be applied at the first layer where input has the desired mesh structure. 


%\paragraph{Applications:}
%It is trendy to develop applications towards using omnidirectional images directly, due to the production of 360\degree images and videos. Applications include image classification \cite{cohen2018spherical}, 3d object classification \cite{cao20173d}, vehicle detection \cite{coors2018spherenet} and saliency localization. \cite{monroy2018salnet360} used 6-patches extracted from omnidirectional image to detect the saliency of 360 images. Perraudin \etal \cite{perraudin2018deepsphere} demonstrate the usage of spherical CNNs on cosmological model classification using maps of projected mass distribution on the sky.

%\section{Method}
%Related to our work in using spherical mesh, Lee \etal \cite{lee2018spherephd} propose to work on icosahedron for spherical convolution and pooling. Instead of representing kernels by triangular faces, we propose to use vertices-based filters while keeping the convolution and pooling simple. The problems we are facing are two-fold: First, we need to determine the order of the ring-1 neighbours so that filters could be applied consistently across all vertices; Second, the design of convolution has to take care of both hexagons and pentagons. First, since we assume the omnidirectional images have a dominant upright orientation, we could place a vertical and horizontal axis at each vertex node, thus ensure the order of the neighbouring nodes. Second, we choose to augment the number of neighbours from 5 to 6 for pentagon nodes, and pad the weight with zero. 
%%% representation
%\subsection{Representation}
%To represent omnidirectional images without introducing distortions, we use spherical mesh (icosahedro as base mesh) as our image representation. Consider equirectangular images as raw inputs, we use the inverse equirectangular projection to project each pixel from image plane to spherical coordinates. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h]
%\centering
%\subfigure[equirectangular]{
%\label{fig:equirect}
%\includegraphics[width=0.5\linewidth]{equirect_image.png}}
%\subfigure[spherical]{
%\label{fig:sphere}
%\includegraphics[width=0.4\linewidth]{sph_image.png}}
%\caption{Equirectangular and spherical representations used in \cite{coors2018spherenet}}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%An example equirectangular image represented using spherical mesh and its triangular geometry is shown in Figure \ref{fig:mesh}.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h]
%\centering
%\subfigure[texture]{
%\includegraphics[trim={2cm, 0, 2.2cm, 0}, width=0.48\linewidth]{pano_sph.png}}
%\subfigure[geometry]{
%\includegraphics[trim={2cm, 0, 2.2cm, 0}, width=0.48\linewidth]{mesh_sph.png}}
%\caption{Our omnidirectional image representation using spherical mesh. Left: with texture; right: triangular mesh geometry.}
%\label{fig:mesh}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% convolution and pooling
%\subsection{Convolution and pooling layer}
%\paragraph{Convolution:}
%A spherical mesh is a collection of triangular faces. Each vertex along with its ring-1 neighbours compose pentagons (5 neighbours) and hexagons (6 neighbours). In order to apply convolution kernels on these vertices, regardless how many neighbours they have, we propose to construct hex-like filters as shown in Figure \ref{fig:convolution_kernel}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h]
%\centering
%\includegraphics[trim={0cm, 0, 0, 0}, width=0.5\linewidth]{hex_kernel.png}
%\caption{Hex-like convolution kernel used in our work. }
%\label{fig:convolution_kernel}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The kernel is considered placing in a canonical orientation with its first element pointing north. To convolve the kernel with arbitrary vertex from spherical mesh, we have to interpolate every vertex together with its neighbours to its canonical form as well. Since the mesh geometry is fixed, the interpolation computation could be done offline. 
%Apart from interpolation weights ($\mathbf{W}$), the neighbours information (indices $\mathbf{K}$ in angular order) also needs to be prepared before convolution could be done. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h]
%\centering
%\subfigure[input]{
%\includegraphics[trim={0cm, 0, 0, 0}, width=0.93\linewidth]{pano_aclzqydjlssfry.jpg}
%}
%\\
%\subfigure[convolution]{
%\includegraphics[trim={0cm, 0, 0, 0}, width=0.45\linewidth]{conv-1.png}
%\label{fig:conv_res}
%}
%\subfigure[max-pooling]{
%\includegraphics[trim={0cm, 0, 0, 0}, width=0.45\linewidth]{pooling-1.png}
%\label{fig:pool_res}
%}
%\caption{Illustration of our convolution and max pooling operations. }
%\label{fig:conv_pool_result}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%To illustrate the effect of applying convolution on spherical meshes, we take an equirectangular image as input and apply a simple sharpening filter. The results are given in Figure \ref{fig:conv_res}. 

%\paragraph{Pooling:}
%Another important operator of this work is pooling layer. Because a spherical mesh could be increased in adjacent levels, pooling layer could therefore become straightforward. That said, max pooling from level $L$ to level $L-1$ only requires keeping the vertices at level $L-1$ while taking the maximum value of each node considering its ring-1 neighbours at level $L$. A sample result applying max pooling is shown in Figure \ref{fig:pool_res}.

% preliminary results
%\section{Preliminary Results}
%\begin{figure}[h]
%    \centering
%    \includegraphics[trim={0cm, 3cm, 0, 0}, clip, width=0.8\linewidth]{mnist.png}
%    \caption{Examples from spherical MNIST}
%    \label{fig:mnist}
%\end{figure}
%To validate the use of spherical mesh for CNNs, we implemented a simple network following Cohen \etal \cite{cohen2018spherical} using spherical MNIST dataset Figure \ref{fig:mnist}. It is composed of two block of convolution-pooling-relu (with 32 and 64 filters, respectively), and one fully connected layers with softmax for classification. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.5]{images/epoch20-bs100.pdf}
%    \caption{Training curve on spherical MNIST}
%    \label{fig:mnist_curve}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The network is trained up to 20 epochs, and the optimizer uses SGD solver with learning rate 0.0001. Figure \ref{fig:mnist_curve} shows the training curve. To compare with state of the art methods, we have a table of accuracy in spherical MNIST Table \ref{tab:mnist_table}. The original experiments proposed in \cite{cohen2018spherical} include three versions that training/test data could be either with random rotation or not. The version shown here is without rotations. Furthermore, Jiang \etal \cite{jiang2018spherical} also propose to move the digits to the equator to avoid coordinate singularity at the poles. 
%\begin{table}[]
%    \centering
%    \begin{tabular}{||c|c||}
%        \hline
%        method &  test err. (\%)\\
%        \hline
%        S2CNN\cite{cohen2018spherical} & 4.00 \\
%        SphereNet\cite{coors2018spherenet} & 5.59 \\
%        PDO CNN\cite{jiang2018spherical} & 0.77 \\
%        Ours & 4.30 \\
%        \hline
%    \end{tabular}
%    \caption{Comparison of accuracy in spherical MNIST}
%    \label{tab:mnist_table}
%\end{table}
%We also wonder how the learned filters look like for the first layer, the visualizations of the 32 filters are shown in Figure \ref{fig:mnist_filters}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.99\linewidth]{filters_layer1.eps}
%    \caption{Visualization of filters in first layer}
%    \label{fig:mnist_filters}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% future work
%\section{Future work}
%Fast semantic segmentation is particular important in self-driving and drone applications, where input is to be parsed quickly to facilitate real-time interactions with the environment. The goal of this work is to propose an efficient and accurate network for omnidirectional images semantic segmentation. Ideally, the network architecture would be suitable for mobile designs due to its significantly reduced number of parameters. 

%To evaluate our method for semantic segmentation task, two datasets are of great interest to us. First, SYNTHIA \cite{ros2016synthia} is a virtual road driving dataset consisting of four video sequences up to a total of 200,000 frames. Images are acquired from a virtual car across different seasons equipped with two multi-cameras. Each multi-cameras includes four monocular cameras with a common center and orientations varying every 90 degrees. Since all cameras have a field of view of 100 degrees, this allows us to extract an omnidirectional version dataset. An example is shown in Figure \ref{fig:synthia_data}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure*}[h]
%    \centering
%    \subfigure[Back]{
%        \includegraphics[width=0.24\linewidth]{dataset_syn/pers/B/000016.png}}
%    \subfigure[Left]{
%        \includegraphics[width=0.24\linewidth]{dataset_syn/pers/L/000016.png}}
%    \subfigure[Front]{
%        \includegraphics[width=0.24\linewidth]{dataset_syn/pers/F/000016.png}}
%    \subfigure[Right]{
%        \includegraphics[width=0.24\linewidth]{dataset_syn/pers/R/000016.png}} \\
%    \subfigure[Omni]{
%        \includegraphics[trim={0cm, 6.5cm, 0, 6.5cm}, clip,width=0.99\linewidth]{dataset_syn/omni/000016.png}
%        \label{fig:synthia_omni}}
%    \subfigure[Label]{
%        \includegraphics[trim={0cm, 6.5cm, 0, 6.5cm}, clip,width=0.99\linewidth]{dataset_syn/color/000016.png}
%        \label{fig:synthia_color}}
%    \caption{Example frame from SYNTHIA dataset. Top: four views taken by monocular cameras; Middle: omni image extracted; Bottom: labels color image}
%    \label{fig:synthia_data}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Another dataset we plan to use is the Stanford 2D3DS dataset \cite{armeni2017joint}. The 2D3DS dataset consists of 1,413 equirectangular images with RGB+depth channels, as well as semantic labels across 13 classes. The panoramic images are taken in 6 different areas. See Figure \ref{fig:2d3ds_data} for a sample. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure*}[h]
%    \centering
%    \subfigure[Omni]{
%        \includegraphics[trim={0cm, 0cm, 0, 0cm}, clip,width=0.99\linewidth]{dataset_2d3ds/omni/camera_0e30c45ea0604ddeb7467fd384362503_office_7_frame_equirectangular_domain_rgb.png}
%        \label{fig:2d3ds_omni}}
%    \subfigure[Label]{
%        \includegraphics[trim={0cm, 0cm, 0, 0cm}, clip,width=0.99\linewidth]{dataset_2d3ds/color/camera_0e30c45ea0604ddeb7467fd384362503_office_7_frame_equirectangular_domain_semantic_pretty.png}
%        \label{fig:2d3ds_color}}
%    \caption{Example frame from Stanford 2D3DS dataset. Top: omni image; Bottom: labels color image}
%    \label{fig:2d3ds_data}
%\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
